TEE-based Selective Testing of Local Workers in Federated Learning Systems

This paper considers a federated learning system composed of a central coordinating server and multiple distributed local workers, all having access to trusted execution environments (TEEs). In order to ensure that the untrusted workers correctly perform local learning, we propose a new TEE-based approach that also combines techniques from applied cryptography, smart contract and game theory. Theoretical analysis and implementation-based evaluations show that, the proposed approach is secure, efficient and practical.

==> basic_design.tex <==

\section{Proposed System Framework}

\subsection{System Components}

We propose a secure federated learning system that has the following roles:
a central server (CS), 
multiple un-trusted local worker (UW);
trusted aggregation agent (TA) co-residing with the CS, and
trusted local monitor (TLM) co-residing with each UW.
Here,
The TA and each TLM are run in TEEs.
When a UW joins the system,
the TLM co-located with the UW should authenticate itself to the CS and the TA.
Then, the TLM should set up secret pairwise keys 
with the UW and the TA, respectively, 
to secure their communications. 
Also, we assume the CS does not collude with any UW.





\subsection{Pre-processing of Local Training Data}

After a UW joins a federated learning system,
it requests its co-located TLM to 
scan all its valid data records and 
process each of them as follows. 

First, 
the TLM assigns a unique identity $i\in [n_R]$ to the record, 
where $n_R$ is the number of such records. 
Thus, each record is denoted as 
\begin{equation}
R_i = \langle i, x_{i,1}, \cdots, x_{i,n_X}, y_i, \cdots, y_{i,n_Y}, \sigma_i \rangle. 
\end{equation}
Second, a Merkle tree for all of the $n_R$ records is built with
$h_i=hash(i|\sigma_i)$ for all $i\in [n_R]$ as leaf nodes. 
The root hash of the tree is denoted as $h_R$.

After the hash tree of all the records has been built as above,
the UW is given the complete Merkle tree while 
the TLM only keeps the Merkle tree root and $n_R$ to itself. 
Following the pre-processing,
the federated learning system runs round by round, where
each round includes the following steps. 





\comment{
the following operations are conducted for each layer.

\item 
The input is tested selectively. and then is used to compute the corresponding output.
Due to the game theoretic analysis, 
the UW should not behave dishonestly; otherwise,
the misbehavior (including faking input or the computation) can be detected.

\item
For each hidden layer, selective testing also works due to the same reasoning as above. 
Particularly, the selective testing is applied on activation function and 
multiplication with matrix (for forward and backward). 
Basically, the operations include: 
    \begin{itemize}
    \item 
    parallel individual operations 
    (evaluation of activation function, back-propagation of activation) - 
    validity of the input's commitment is checked selectively, 
    computation is selectively repeated, and 
    validity of the output's commitment is checked selectively;
    \item
    parallel matrix operations
    (linear combination of inputs for a convolutional or fully connected layer, and 
    the corresponding back-propagation) -
    select the computations to check, 
    the input elements of the selected computation are retrieve and the elements are selectively checked,
    computation is selectively repeated, and
    validity of output is checked selectively;
    \item 
    summation 
    (occurring in the forward and backward propagation of convolutional layer) - 
    the summation is organized in a hierarchy, 
    validity of each layer's commit is checked selectively, 
    the computation is selectively repeated, and 
    validity of output's commitment is checked selectively;
    \item 
    computation of the cost/loss function - 
    directly repeat the computation (due to the small scale).
    \end{itemize}

\item 
Challenge with convolutional layer back-propagation: update on a weight is a sum of a large number of mini-updates; 
how to test summation efficiently? Answer - hierarchical approach; that is, one sum is treated as the sum of a certain number of sub-sums, where
each sub-sum is further treated as a certain of even lower-level sub-sums, and so on and so forth. 
Game theoretic approach plus selective testing can then be applied on each layer to verify. (Interesting design!)

}








\subsection{Initializing Each Round (a.k.a. Testing for Layer~1)}

For the simplicity of presentation, 
we assume that only one record is processed in each round. 
At the beginning of a round, 
the TLM randomly selects an ID $i\in [n_R]$, 
and asks the UW to pick the record with the ID for training. 

In response, 
the UW retrieves the content of the selected record (i.e., $R_i$), 
the record hash (i.e., $h_i=hash(i|\sigma_i)$), and 
the corresponding co-path hash values on the Merkle tree of all $n_R$ records.
Then, it communicates $h_i$ and the corresponding co-path hash values,
which are called the {\em commitment} of the input,
to the TLM.

Upon receiving the commitment,
the TLM verifies it by recomputing the root hash with $h_i$ and its corresponding co-path hash values
and checking if the recomputed root hash is the same as $h_R$. 
Once, the verification succeeds, 
the TLM records the commitment and proceeds with the rest of the round;
otherwise, it identifies the UW as dishonest and stops the process. 




\subsection{Testing for Each Hidden Layer}

At each hidden layer $l$,
both forward and backward propagation through it should be tested.

For the forward propagation, 
the output from the previous layer $l-1$ is first transformed,
e.g., through a fully-connected network or a set of filter matrices, 
to the input of the neurons of layer $l$; then,
at each neuron, an activation is applied on the input element 
to obtain the corresponding output element. 
Selective testing for the transformation is complex and thus 
we leave the detail of it to Section~\ref{}. Here,  
we only elaborate the testing for 
the activation function as follows.
\begin{itemize}

\item 
Before the evaluation of activation function starts,
the UW should have already computed and submitted to the TLM 
a commitment of the input to layer $l$, denoted as $Commit(I_l)$,
which is the root of the Merkle hash tree 
with the hashes of the input elements as leaf nodes. 

\item 
For each neuron at layer $l$,
the input element is fed to the activation function 
and the corresponding output element is obtained.
Then, the UW constructs a Merkle hash tree 
with the hashes of these output elements as leaf nodes.
The root of this tree, denoted as $Commit(O_l)$, 
is called the commitment of the output, 
and should be submitted to the TLM. 

\item 
The TLM randomly selects $i\in [n_l]$ and requests the UW to 
send the $i$-th input and output elements, 
along with their corresponding co-path hash values on 
their respective input and out Merkle hash trees.
Upon receiving the above,
the TLM recomputes the roots of the two Merkle hash trees,
and verify if the recomputed root hashes 
are the same as $Commit(I_l)$ and $Commit(O_l)$, respectively. 
If the verification succeeds, 
the testing for the activation function also succeeds;
otherwise, the TLM identifies the UW as dishonest 
and evicts it from the system.  
\end{itemize}

For the backward propagation,
the gradients for the output elements of layer $l$ 
should have been computed by the UW 
when the backward propagation was conducted through layer $l+1$.
Also, the commitment for these gradients should have been 
computed and submitted by the UW to the TLM.
First, the TLM conducts selective testing for the backward propagation of 
gradients from the output of the activation function to the input of the function.
Specifically, it is as follows.
    The UW computes the gradients of the input of the activation function
    from the gradients of the output. Then,
    the UW computes the commitment for the gradients of the input
    and sends it to the TLM. 
    Upon receiving the commitment,
    the TLM randomly selects $i\in [n_l]$,
    requests the UW to return the gradients for the $i$-th output and input elements of the activation function
    along with their corresponding co-path hashes on the Merkle trees.  
    
Second, the TLM conducts selective testing for 
the backward propagation from the input of layer $l$ to the output of layer $l-1$
and also the computation of updates to the transformation matrices between the two.
The detail for this step is explained in Section~\ref{}
for the cases that the transformation is a fully-connected network
and that it is a set of filters. 


















\subsection{Testing Forward Propagation}

\subsubsection{Testing Input to Fully-connected Layer}

For a fully-connected hidden or final layer $l$,
it takes vector $\vec{O}_{l-1}$, 
the $n^{(l-1)}_O$ elements outputted by layer $l-1$,
and left-multiplies it with a matrix of weights, 
$\Theta^{(l)}$, which has $n^{(l)}_I$ rows and $n^{(l-1)}_O$ columns,
to obtain its input vector $\vec{I}_{l}$ of $n^{(l)}_I$ elements. 


At this point, 
the TLM should have validated the computation of $\vec{O}_{l-1}$;
that is, the commitment $commit(\vec{O}_{l-1})$ has already been validated.
To facilitate the TLM's testing of the above operation,
the UW should compute a commitment as follows:
\begin{itemize}
    \item
    The UW constructs a Merkle tree with the elements in $\vec{I}_{l}$ as leaf nodes.
    \item
    The UW submits to the TLM the root of the above Merkle tree, 
    denoted as $commit(\vec{I}_{l})$, 
    which serves as the commitment.    
\end{itemize}

To test the above operation,
the TLM acts as follows.

First, the TLM obtains $\vec{O}_{l-1}$ from the UW and tests the validity of this obtained version. 
Specifically, it randomly picks $\alpha$ elements of the vector, 
requests the corresponding co-path values for these elements,
and tests the validity of these elements by checking 
if $commit(\vec{O}_{l-1})$ can be re-computed. 


Second, the TLM tests the validity of the computation as follows.
\begin{itemize}
    \item 
    It randomly picks $\alpha$ rows of $\Theta^{(l)}$,
    and multiple these rows with $\vec{O}_{l-1}$ respectively.
    Specifically, letting the randomly picked rows be $i_1, \cdots, i_{\alpha}$, 
    the results are 
        \begin{equation}
            r_j = (\theta_{1,j}, \cdots, \theta_{n^{(l-1)}_O,j})\cdot\vec{O}_{l-1},
        \end{equation}
    for $j=1,\cdots,\alpha$.
    \item 
    It checks if the results are the corresponding elements of the committed input vector. 
    Specifically, for each $j=1,\cdots,\alpha$,  
    it requests the UW to return the co-path values for leaf node $r_j$ on the Merkle tree;
    if the Merkle tree root computed with the co-path values equals to the committed $commit(\vec{O}_{l-1})$,
    $r_j$ is validated. 
    Only if all the $\alpha$ results are validated, 
    the committed input vector is validated. 
\end{itemize}











\comment{
TA should prepare and send some information to each TLM which is co-located with a local worker,
to facilitate the TLM's work. 


Initially, each UW is preloaded with an initial model of neural network.

Then, after every round of distributed learning,
the TA provides the aggregated cost to each UL securely (i.e., without being modified);
based on the cost, each UL updates its model by updating the weights of edges on the neural network model.

The URM can also update the model synchronously with each UL.
Then, the URM and each TLM collaborate to verify the learning procedure at the UL that the TLM co-resides with.
The URM should pre-share the following keys with each TLM:
\begin{itemize}
\item
a symmetric key; and
\item
a pair of public/private key for partial homomorphic encryption (PHE) such as the Paillier cryptosystem.
\end{itemize}
For each layer $l$, the URM prepares material for verification purpose
and share them with either TLMs or ULs, as follows:
\begin{itemize}

\item
It randomly generates a vector $\vec{s}_l$ of $O_l$ elements and
computes $\vec{s'}_l\leftarrow \vec{M}_l\times \vec{s}_j$.

\item
Let $\alpha\in (0,1)$ be a system parameter.
$q_l=\lceil I_l\cdot\alpha \rceil$ and
$q_{l+1}=\lceil O_{l}\cdot\alpha\rceil$.
The URM processes $\vec{s}_l$ and $\vec{s'}_l$ respectively as in the following.

\item
the URM randomly selects $q_l$ elements from $\vec{s}_l$ to form set ${\cal S}_0$
while the rest elements of $\vec{s}_l$ form set ${\cal S}_1$:
    \begin{itemize}
    \item
    All the elements in ${\cal S}_0$, along with their indices in $\vec{s}_l$
    should be securely sent to each TLM (without being exposed to the UL).
    \item
    For each element $s_j$ in $S_1$, it is encrypted to $c_j = PHE(s_j)$
    Note that, the encryption conducted by $PHE$ uses a pair of public key and private key,
    where the private key is known only by the URM and each TLM but
    the public key is shared with each UL.
    The encrypted elements of ${\cal S}_1$ are further encrypted with a randomly-selected symmetric key
    and these double-encrypted elements (along with their indices on vector $\vec{s}_l$) should be shared with the UL.
    \item
    The randomly-selected symmetric key used in the second tier of encryption is encrypted with the symmetric key shared
    between the TA and each TLM; the encrypted key is then shared with each TLM.
    \end{itemize}


\item
Vector $\vec{s'}_l$ is processed similar to the above.
the URM randomly selects $q_{l+1}$ elements from $\vec{s'}_l$ to form set ${\cal S}'_0$
while the rest elements of $\vec{s'}_l$ form set ${\cal S}'_1$.
    \begin{itemize}
    \item
    All the elements in ${\cal S}'_0$, along with their indices in $\vec{s}'_l$
    should be securely sent to each TLM (without being exposed to the UL).
    \item
    For each element $s'_j$ in $S'_1$, it is encrypted to $c'_j = PHE(s'_j)$
    The encrypted elements of ${\cal S}'_1$ are further encrypted with the secret symmetric key shared between the URM and each TLM,
    and these double-encrypted elements (along with their indices on vector $\vec{s}'_l$) should be shared with the UL.
    \item
    The randomly-selected symmetric key used in the second tier of encryption is encrypted with the symmetric key shared
    between the TA and each TLM; the encrypted key is then shared with each TLM.
    \end{itemize}



\end{itemize}
}



\subsubsection{Testing Input to Convolutional Layer}

For a convolutional hidden layer $l$,
each input element is computed as the inner product between 
a filter vector (or matrix) and 
a sub-vector of the output vector (or matrix) of layer $l-1$.

Before the above computation, 
the commitment of the layer $l-1$'s output vector $\vec{O}_{l-1}$ should have already been validated.
To facilitate validating the above computation, 
the UW should commit the layer $l$'s input vector $\vec{I}_l$.
This is accomplished by constructing a Merkle tree with the elements of $\vec{I}_l$ as leaf nodes,
and treating the root of the tree, denoted as $commit(\vec{I}_l)$, as the commit. 

The validation of the above computation is conducted by the TLM as follows.
The TLM randomly picks $\alpha$ sub-vectors from $\vec{O}_{l-1}$, 
multiply them with their corresponding filter vectors respectively, 
and obtain the $\alpha$ results.
The results should be the same as their corresponding elements in $\vec{O}_l$. 
To verify this, for each of the $\alpha$ results,
the TLM requests the UW to provide the corresponding co-path values on the Merkle tree
to re-compute the root of the tree.
If the re-computed root is the same as $commit(\vec{I}_l)$ for all the $\alpha$ cases,
the validation succeeds; otherwise, it fails. 














\subsubsection{Testing Loss Function Computation}

At the end of forward propagation, 
the UW feeds the elements of input and y-vector (i.e., $(y_{i,1}, \cdots, y_{i,n_Y})$) to the loss function to obtain the value of loss,
and submits the value to the TLM.
Because the number of input elements is usually small,
the TLM tests the computation by directly re-computing the value of loss, as follows.google.com/google.com/
google.com/%
\begin{itemize}
\item 
First, the TLM requests the UW to obtain all the elements of input and y-vector.
\item 
Second, the TLM tests the validity of the obtained input elements and y-vector through selective testing. 
Specifically, it randomly picks $\alpha$ input elements and $\alpha$ elements of the y vector;
for each of the picked elements,
it requests the UW for the corresponding co-path values;
based on the hash of the picked elements and the co-path values, it re-computes the root of Merkle tree;
this step succeeds only if the re-computed root is the same as the commitment submitted by the UW earlier for all the $2\alpha$ cases.
\item 
Third, the TLM re-computes the value of loss by feeding the obtained input elements and y-vector to the loss function,
and compares the re-computed value with the value of loss submitted by the UW.
\end{itemize}




\subsection{Testing Backward Propagation}

In the beginning of backward propagation,
the UW computes the gradients for the inputs of the loss function.
To commit the computation, 
the UW constructs a Merkle tree with the hashes of these gradients as leaf nodes,
and submits to the TLM the root of the Merkle tree as commitment. 
To test the computation, 
the TLM re-computes the gradients, 
re-constructs the Merkle tree, and 
checks if the root of the re-constructed Merkle tree is the same as the commitment. 

\subsubsection{Testing Backward Propagation through Fully-connected Layer}

Before the UW conducts backward propagation at a fully-connected layer $l$,
the gradients for the outputs of the layer's activation functions should 
have already been computed and committed. 

The UW conducts backward propagation as follows. 
\begin{itemize}
    \item 
    It computes the gradients for the inputs of the activation functions,
    constructs a Merkle tree with the hashes of these gradients as leaf nodes,
    and submits to the TLM the root of the Merkle tree as the commitment of these gradients.
    \item 
    For each pair of $(i,j)$ where $i$ is the index of input at layer $l$ and $j$ is the index of output at layer $l-1$,
    letting $\nabla i$ denote the gradient for input $i$ and $o_j$ denote the value of output $j$,
    weight the update for $\theta^{(l)}_{i,j}$, 
    denoted as $\Delta\theta^{(l)}_{i,j}$, 
    is computed as $-\eta\cdot\nabla i\cdot o_j$.
    \item 
    It multiplies the gradients with the transpose of $\Theta^{(l)}$, 
    to obtain the gradients for the outputs of layer $l-1$.
    \item 
    The UW computes and submits to the TLM the commitments for
    (i) the input gradients of layer $l$,
    (ii) the updates to all weights in $\Theta^{(l)}$, and 
    (iii) the output gradients of layer $l-1$.
\end{itemize}

After receiving the commitments,
the TLM conducts selective testing of the backward propagation, as follows. 
\begin{itemize}
    \item 
    It retrieves the gradients of all the inputs to activation functions of this layer.
    Then it conducts the following checking step by step. 
    If a checking fails, the UW is found dishonest; otherwise, the checking continues. 
    \item 
    It randomly selects $\alpha$ output gradients of layer $l$ to retrieve from the UW. 
    Based on the submitted commitment for these output gradients,
    it verifies the validity of the selected gradients.
    \item 
    Based on the selected output gradients and the activation functions,
    the TLM re-computes the gradients of their corresponding inputs. Then, 
    checking is done in two aspects:
    the re-computed gradients should be consistent with those retrieved 
    the validity of these input gradients are verified based on the submitted commitment for them.
    \item 
    The TLM randomly selects $\alpha$ rows of matrix $\Theta^{(l)}$ to obtain a sub-matrix. 
    The sub-matrix is multiplied with the vector of all of the inputs of layer $l$,
    resulting in $\alpha$ gradients of output of layer $l-1$.
    The validity of each of these $\alpha$ outputs is checked based on the submitted commitment for the outputs.
    \item 
    The TLM retrieves from the UW $\alpha$ updates on weights that are randomly selected.
    For each of these update, denoted as $\Delta\theta^{(l)}_{i,j}$,
    it computes output $o_j$ of layer $l-1$ as $o_j=\frac{\Delta\theta^{(l)}_{i,j}}{\nabla i}$ and 
    checks the validity of $o_j$ based on the commitment submitted by the UW for the ouputs of layer $l-1$.
\end{itemize}


\subsubsection{Testing Backward Propagation through Convolutional Layer}

Before the UW conducts backward propagation at a convolutional layer $l$,
similar to the case of fully-connected layer, 
the gradients for the outputs of the layer's activation functions should 
have already been computed and committed. 

The UW conducts the backward propagation as follows.
\begin{itemize}
    \item 
    It computes the gradients for the inputs of the activation functions
    (denoted as $\nabla\vec{I}_i$ for $i=n_I$ where $n_I$ is the size of inputs),
    constructs a Merkle tree with the hashes of these gradients as leaf nodes,
    and submits to the TLM the root of the Merkle tree as the commitment of these gradients.
    
    \item 
    It computes the gradients for the output of layer $l-1$ and for the elements of filter matrices.
    Specifically, the computation is as follows.
    \begin{itemize}
        \item
        For each input element $\vec{I}_i$,
        let $\vec{I}_i$ be computed as the inner product of 
        filter $\vec{F}$ (a vector of $|\vec{F}|$ elements)
        and vector $\vec{O}$ ($\vec{F}$ output elements of layer $l-1$'s output).
        \item
        For each $j\in [|\vec{F}|]$,
        $\nabla\vec{O}_j += \nabla\vec{I}_i\cdot\vec{F}_j$ and 
        $\nabla\vec{F}_j += \nabla\vec{I}_i\cdot\vec{O}_j$.
    \end{itemize}
    
    \item
    It computes the commitments. 
    For the gradients for the output of layer $l-1$,
    the UW constructs a Merkle tree with the hashes of these gradients as leaf nodes. 
    For the gradients for the filters,
    the UW also constructs a Merkle tree with the hashes of these gradients as leaf nodes. 
    The roots of these Merkle trees are submitted to the TLM as commitments. 
    
    \item 
    The cost for re-computing the gradients of filters may be high. 
    The cost can be reduced with the following technique. 
    For each filter matrix $\vec{F}$,
    all the input elements of layer $l$ whose computation involves $\vec{F}$ are divided into $g$ groups. 
    For each of such groups, 
    group-gradients of the filter elements are computed only based on the gradients of the outputs in the group.
    A modified hash tree is built for each filter element with the group-gradients computed as above. 
    When checking one filter gradient,
    the TLM does not re-compute the gradient;
    instead, it retrieves the hash tree, and only compute $\alpha$ leaves of the tree and verify 
    using the technique similar to that for Merkle hash tree. 
    
    
    \comment{
    \item 
    For each pair of $(i,j)$ where $i$ is the index of input at layer $l$ and $j$ is the index of output at layer $l-1$,
    letting $\nabla i$ denote the gradient for input $i$ and $o_j$ denote the value of output $j$,
    weight the update for $\theta^{(l)}_{i,j}$, 
    denoted as $\Delta\theta^{(l)}_{i,j}$, 
    is computed as $-\eta\cdot\nabla i\cdot o_j$.
    \item 
    It multiplies the gradients with matrix $\Theta^{(l)}$, 
    to obtain the gradients for the outputs of layer $l-1$.
    \item 
    The UW computes and submits to the TLM the commitments for
    (i) the input gradients of layer $l$,
    (ii) the updates to all weights in $\Theta^{(l)}$, and 
    (iii) the output gradients of layer $l-1$.
    }
    
    
\end{itemize}









\comment{
\subsection{Training and Associated Committing Process}

For each round, at each UL for each set of input,
the input is processed through the network until the cost function is computed,
which is the same as a regular training process.

Along with the above training process,
the UL also does the following to make records for the purpose of proving itself (or being verified by its co-residing TLM).
During the processing of each set of input, at each layer $l$,
the UL constructs a Merkel hash tree with the input elements as leaf nodes;
it also constructs a Merkel hash tree with the output elements as leaf nodes.
The root values of these Merkel hash trees should be shared with the TLM immediately after they have been computed.

\subsection{TLM-UL Interaction: Proofing and Verification}

After a round of training has been completed, each TLM interacts with its co-residing UL as follows to verify the training process.

First, Each TLM shares with its co-residing UL the encrypted symmetric key,
which is used by the UL to decrypt the preloaded material for the proofing/verification purpose.

Then, for each input set processed by the UL, the proofing/verification is conducted as follows.

\subsubsection{Verifying the Input Set}

Each input set is endorsed by a signature generated by a trusted entity whose public key is known in the public domain.
Particularly, the signature is over the root of a Merkel hash tree
with the elements of the input set as leaf nodes.

When verifying the inputs of the first layer,
the TLM randomly selects a subset of input elements,
and requests the UL to provide these selected elements
along with their co-path elements on the Merkel hash tree.
Then, the validity of these selected elements can be verified by
checking if they together with their co-path elements
can be computed to a root of the Merkel tree whose signature is valid.


\subsubsection{Verifying the outputs of each layer}

For each layer $l$, the UL is already preloaded with:
\begin{itemize}
\item
${\cal S}_l$ (i.e., a subset of elements in $\vec{s}_l$ that have been encrypted with PHE)
along with these elements' indices in the vector;
assume they are denoted as
\[
(j_1, \hat{s}_{j_1}), (j_2, \hat{s}_{j_2}), \cdots, (j_x, \hat{s}_{j_x})
\]
where each $j_t$ is index and $\hat{s}_{j_t}=PHE(s_{j_t})$ is the encrypted element in $\vec{s}_l$.
\item
${\cal S}'_l$ (i.e., a subset of elements in $\vec{s}'_l$ that have been encrypted with PHE)
along with these elements' indices in the vector;
assume they are denoted as
\[
(j'_1, \hat{s'}_{j'_1}), (j'_2, \hat{s'}_{j'_2}), \cdots, (j'_y, \hat{s'}_{j'_y})
\]
where each $j'_t$ is index and $\hat{s'}_{j_t}$ is the encrypted element in $\vec{s'}_l$.
\end{itemize}

Then, the UL computes the following:
\[
\hat{A}_l = \sum_{t=1}^{x} i_{j_t}\cdot\hat{s}_{j_t},
\]
where $i_{j_t}$ is an element in $\vec{i}_l$ at index $j_t$;
\[
\hat{A'}_l = \sum_{t=1}^{y} o_{j'_t}\cdot\hat{s'}_{j'_t},
\]
where $o_{j'_t}$ is an element in $\vec{o}_l$ at index $j'_t$.

The computed $\hat{A}_l$ and $\hat{A'}_l$ are provided to the co-residing TLM,
which decrypts them to $A_l$ and $A'_l$.

Recall that the TLM is preloaded with
\[
(j_{x+1}, s_{j_{x+1}}), \cdots, (j_{i_l}, \hat{s}_{j_{i_l}})
\]
and
\[
(j'_{y+1}, s'_{j'_{y+1}}), \cdots, (j'_{o_l}, \hat{s'}_{j'_{o_l}}).
\]

Then, the TLM computes the following:
\[
B_l = \sum_{t=x+1}^{i_l} i_{j_t}\cdot s_{j_t},
\]
and
\[
B'_l = \sum_{t=y+1}^{o_l} o_{j'_t}\cdot s'_{j'_t}.
\]

The TLM then checks if the following condition is satisfied:
\[
A_l + B_l = A'_l + B'_l.
\]

Once the above condition is satisfied,
the TLM randomly picks some elements in ${\cal S}_0$ and ${\cal S}_1$ and check their validity
by checking if they are leaf nodes of the Merkel hash trees whose roots have been committed already.




\subsubsection{Verifying the inputs of each non-first layer}

To verify the validity of inputs on layer $l+1$ given the outputs of layer $l$,
each TLM does the following.

The TLM randomly selects a subset of elements from the outputs of layer $l$
and their corresponding elements in the inputs of layer $l+1$.
It is verified that each of the selected output element of layer $l$
is correctly converted to its corresponding input element of layer $l+1$.

If the above is correct,
the TLM further checks if the selected elements are leaf nodes of the Merkel trees
whose roots have been committed in the earlier training and committing step.




\subsubsection{Verifying the computation of cost function}

To verify the computation of cost functions,
the TLM simply repeat that. As the number of elements for final output is typically small,
this should not be a significant overhead.
}

==> details.tex <==

\section{Enhancements for Higher Efficiency}


In this section, 
we present the detailed designs for 
testing the forward/backward propagation through 
the transformation stages at convolutional or fully-connected layer $l$.
Several enhancements for efficiency are included. 

\subsection{Convolutional Layer: Forward Propagation}
\label{sec:conv-forward-detail}

The general model presented in Section~\ref{sec:select-test-general-model}
may be directly applied for the testing. However, 
when the sizes of $\vec{X}$ and/or $\vec{Y}$ are large, 
the costs for the UW to compute the Merkle trees and 
for the TLM to conduct selective testing could be very high. 
To address this problem,
we propose the following more-efficient scheme. 

\subsubsection{Computations by the UW}

If being honest, the UW first computes $\overrightarrow{Y}$ 
according to Equation~(\ref{eq:conv-forward})
in Section~\ref{sec:conv-basic}.
Then, it constructs hash trees for $\vec{X}$ and $\vec{Y}$ as follows. 

To construct a hash tree for $\vec{X}$,
the matrix $\vec{X}$ is first divided into sub-matrices 
$\{\vec{X}_{i,j} | i,j\in[\beta_X]\}$ such that, 
each sub-matrix $\vec{X}_{i,j}$ contains elements 
$\{\vec{X}[u,v]|u=(i-1)\cdot\alpha'_F+1,\cdots, \min(i\cdot\alpha'_F,\alpha_X); u=(j-1)\cdot\alpha'_F+1,\cdots, \min(j\cdot\alpha'_F,\alpha_X)\}$ where $\alpha'_F=\delta\cdot\lceil\frac{\alpha_F}{\delta}\rceil\geq\alpha_F$.
We call these sub-matrices as {\em landmark} sub-matrices.
For each {\em landmark} sub-matrix $\vec{X}_{i,j}$,
a hash value $h(\vec{X}_{i,j})$ is computed as 
the hash of all the elements belong to it.
Finally, a Merkel hash tree is constructed with all these hash values
as the leaf node; the tree is denoted as $tree(\vec{X})$ and
the root of the tree is denoted as commitment $comm(\vec{X})$.

To construct a hash tree for $\vec{Y}$, %
a hash for each row $r\in[\alpha_Y]$ of 
$\overrightarrow{Y^{(t)}}$ for $t\in[n_F]$ is computed and 
denoted as $h(\overrightarrow{Y^{(t)}}[r])$.
Then, a hash tree is constructed with all these hash values as leaf nodes;
the tree is denoted as $tree(\vec{Y})$ and
the root of the tree is denoted as commitment $comm(\vec{Y})$.

After the above hash trees have been constructed,
the UW sends $comm(\vec{X})$ and $comm(\vec{Y})$ to the TLM. 




\subsubsection{Selective Testing by the TLM}


The UW provides the following information to the TLM:
\begin{itemize}
    \item filter $\overrightarrow{F^{(t)}}$ for each $t\in[n_F]$
        along with the signature for it signed by the CS,
        denoted as $\sigma(CS,\overrightarrow{F^{(t)}})$;
    \item the pointers to the memory spaces where 
        $\overrightarrow{X}$,
        $\overrightarrow{Y}$,
        $tree(\overrightarrow{X})$ and 
        $tree(\overrightarrow{X})$ 
        are stored respectively.    
\end{itemize}
Upon receiving the above information,
the TLM randomly selects $p$ elements of $\overrightarrow{Y}$ to test.
For each of the selected element, denoted as $\overrightarrow{Y^{(t)}}[i,j]$,
the testing is conducted as follows.\\

{\noindent \em [Test~1]}:~ 
It is verified whether $\sigma(CS,\overrightarrow{F^{(t)}})$ 
is a valid signature for $\overrightarrow{F^{(t)}}$ generated by the CS.\\

{\noindent \em [Test~2]}:~
First, a sub-matrix $\overrightarrow{X'}$ of $\vec{X}$ is identified
to contain the elements are used in computing $\overrightarrow{Y^{(t)}}[i,j]$.
According to Equation~\ref{eq:conv-forward},
$\overrightarrow{X'}$ includes 
$\vec{X}[u,v]$ for all 
$(i-1)\delta+1\leq u\leq(i-1)\delta+\alpha_F$ 
and $(j-1)\delta+1\leq v\leq(j-1)\delta+\alpha_F$.

Second, the landmark sub-matrices that cover all the elements of $\overrightarrow{X'}$ are identified.
According to the definition of landmark sub-matrices,
$\overrightarrow{X'}$ is covered by the following landmark sub-matrices:
$\vec{X}_{u',v'}$, $\vec{X}_{u',v'+1}$, $\vec{X}_{u'+1,v'}$ and $\vec{X}_{u'+1,v'+1}$,
where $u'=\alpha'_F\cdot\lceil\frac{i}{\alpha'_F}\rceil+1$ and 
$v'=\alpha'_F\cdot\lceil\frac{j}{\alpha'_F}\rceil+1$.

Third, the elements in the afore-identified landmark-matrices are retrieved,
and the validity of these elements is checked based on $Tree(\vec{X})$ as follows.
For each landmark sub-matrix,
the hash of all the elements in it is computed, and 
the computed hash (denoted as $h$) should be equal to 
the leaf node with a corresponding index (denoted as $i$) in $Tree(\vec{X})$.
Then, the co-path values of the leaf node are retrieved to form evidence $e$
and $Verify_Commit(h,i,comm(\vec{X}),e)$ is called to verify the validity.\\

{\noindent \em [Test~3]}:~
The values for row $\overrightarrow{Y^{(t)}}[i]$ are retrieved, and 
its validity is verified based on $Tree(\vec{Y})$ as follows (similarly to Test~2).
The hash of all the elements in the retrieved row is computed,
and the computed hash (denoted as $h'$) should be equal to 
the leaf node with a corresponding index (denoted as $i'$) in $Tree(\vec{Y})$.
Then, the co-path values of the leaf nodes are retrieved to form evidence $e'$
and finally $Verify_Commit(h',i',comm(\vec{Y}),e')$ is called to verify the validity.

{\noindent \em [Test~4]}:~
Lastly, it is checked whether $\overrightarrow{X'}\cdot\overrightarrow{F^{(t)}}$ is equal to
$\overrightarrow{Y^{(t)}}[i][j]$ retrieved in the previous step. \\

{\noindent If} any of the above tests fails,
the TLM identifies the UW as dishonest and stops working with the UW.
Otherwise, the selective testing succeeds. 












\subsection{Convolutional Layer: Backward Propagation}

During the backward propagation,
the UW could compute the gradients for $\vec{X}$ 
according to Equation~(\ref{eq:conv-backward})
based on $\overrightarrow{\nabla Y}$ and the filters;
compute the updates to every filter 
according to Equation~(\ref{eq:conv-update})
based on $\overrightarrow{\nabla Y}$ and $\vec{X}$.
To facilitate selective testing efficiently,
however, changes need to be made to the above procedure. 
We elaborate the new computation procedure and 
the selective testing of the above computation in the following.

\subsubsection{Computation by the UW}


To facilitate selective test,
the TLM should record some intermediate results of the computations 
and construct several hash trees. \\ 

{\noindent\bf\underline{Computation of 
$\overrightarrow{\nabla X}$ and $Tree(\overrightarrow{\nabla X})$}}:
For each filter $\overrightarrow{F^{(t)}}$ for $t\in[n_F]$,
the TLM computes a matrix $\overrightarrow{\nabla X^{(t)}}$
based on Equation~(\ref{eq:conv-backward-1}); then,
it computes matrix $\overrightarrow{\nabla X}$ based on Equation~(\ref{eq:conv-backward}).

After the above computation, 
the TLM records both $\{\overrightarrow{\nabla X^{(t)}}|t\in[n_R]\}$ and 
$\overrightarrow{\nabla X}$.
Also, it constructs a Merkle hash tree $Tree(\overrightarrow{\nabla X})$
based on $\{\overrightarrow{\nabla X^{(t)}}|t\in[n_R]\}$.
Specifically,
for each $i,j\in[\alpha_X]$,
the TLM computes $h(\overrightarrow{\nabla X},i,j)$ as
$hash(\overrightarrow{\nabla X^{(1)}}[i,j],\cdots,\overrightarrow{\nabla X^{(n_F)}}[i,j])$,
all these hash values are used as leaf nodes to construct $Tree(\overrightarrow{\nabla X})$,
and the root of the tree is denoted as commitment $comm(\overrightarrow{\nabla X})$.\\

{\noindent\bf\underline{Computation of 
$\overrightarrow{\nabla F^{(t)}}$ and $Tree(\overrightarrow{\nabla F})$}}:
To record some intermediate results of computing $\overrightarrow{\nabla F^{(t)}}$, 
Each element of it, i.e., 
$\overrightarrow{\nabla F^{(t)}}[i,j]$ for every $i,j\in[\alpha_F]$, 
is expanded to a $\alpha_Y$-element vector
denoted as $\overrightarrow{\nabla F^{(t)}_{i,j}}$. Specifically,
each element of $\overrightarrow{\nabla F^{(t)}_{i,j}}$,
which is denoted as $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$ for $u\in[\alpha_Y]$,
is computed as
\begin{equation}\label{eq:nabla_Ft_iju}
    \overrightarrow{\nabla F^{(t)}_{i,j}}[u]=
        \sum_{v\in[\alpha_Y]} \overrightarrow{\nabla Y^{(t)}}[u,v]\cdot \vec{X}[(u-1)\alpha_F+i,(v-1)\alpha_F+j].
\end{equation}
Then, $\overrightarrow{\nabla F^{(t)}}[i,j]$ is computed as
\begin{equation}
    \overrightarrow{\nabla F^{(t)}}[i,j] = 
    \sum_{u\in [\alpha_Y]}\overrightarrow{\nabla F^{(t)}_{i,j}}[u].
\end{equation}
For each vector $\overrightarrow{\nabla F^{(t)}_{i,j}}$ for $t\in [n_F]$ and $i,j\in[\alpha_Y]$,
the hash of all its elements is computed.
Then all these hash values for every $t$, $i$ and $j$
are used as leaf node to construct Merkel hash tree
$Tree(\overrightarrow{\nabla F})$. \\

{\noindent\bf\underline{Construction of 
$Tree(\overrightarrow{\nabla Y})$ and $Tree'(\overrightarrow{X})$}}:
Based on how $\overrightarrow{\nabla Y}$ and $\overrightarrow{X}$
are used in the above Equation~(\ref{eq:nabla_Ft_iju}),
the TLM further construct the following two Merkel hash trees.

For each $t\in[n_F]$, a hash value is computed for 
all the $\alpha_Y$ elements of each row of $\overrightarrow{\nabla Y^{(t)}}$.
Then, all these $\alpha_Y\cdot n_F$ hash values are used as leaf nodes
to construct Merkel hash tree $Tree(\overrightarrow{\nabla Y})$.

For each $i,j\in[\alpha_F]$ and each $u\in[\alpha_Y]$,
we define a group denoted as $\vec{X}_{i,j,u}$ that includes 
the following elements of $\vec{X}$: 
$\vec{X}[(u-1)\alpha_F+i,(v-1)\alpha_F+j]$ for every $v\in[\alpha_Y]$.
The hash for all the elements in $\vec{X}_{i,j,u}$, 
denoted as $h(\vec{X}_{i,j,u})$, is computed.
Then, all of the above hash values  
$h(\vec{X}_{i,j,u})$ for every $u\in[n_F]$
are used as leaf nodes to construct Merkel hash tree $Tree'(\overrightarrow{X})$.



\subsubsection{Selective Testing by the TLM}

Similar to the forward propagation, 
the UW also provides the following information to the TLM:
(i) each filter and its signature; 
(ii) the pointers to the memory spaces where 
$\vec{X}$, 
$\overrightarrow{\nabla Y}$, 
$\overrightarrow{\nabla F}$, 
$\overrightarrow{\nabla X}$,
$\overrightarrow{\nabla X^{(t)}}$ for every $t\in[n_F]$,
$Tree'(\vec{X})$, 
$Tree(\overrightarrow{\nabla Y})$,
$Tree(\overrightarrow{\nabla F})$, and 
$Tree(\overrightarrow{\nabla X})$.
After receiving the above information,
the TLM verifies the validity of the filters, and then
selectively tests the computations of
$\overrightarrow{\nabla X}$ and 
$\overrightarrow{\nabla F}$.

{\noindent\bf\underline{Selective Testing of $\overrightarrow{\nabla X}$}}:
The TLM randomly selects $p$ elements of $\overrightarrow{\nabla X}$ to test.
For each of the selected element,
denoted as $\overrightarrow{\nabla X^{(t)}}[i,j]$ for 
some $t\in[n_R]$ and $i,j\in[\alpha_X]$, 
the testing is as follows.

{\noindent\em [Test~1]}:~
The validity of $\overrightarrow{\nabla X^{(t)}}[i,j]$ is verified 
based on $Tree(\overrightarrow{\nabla X})$.
Specifically, a hash value is computed as 
$h=hash(\overrightarrow{\nabla X^{(1)}}[i,j],\cdots,\overrightarrow{\nabla X^{(n_F)}}[i,j])$;
it is checked whether $h$ equals to the leaf node of $Tree(\vec{X})$
at the corresponding position $ind$;
the co-path values of the leaf node are retrieved from $Tree(\vec{X})$ to form evidence $evid$;
$Verify\_Commit(h,ind,comm(\vec{X}),evid)$ is called to verify the validity. 


{\noindent\em [Test~2]}:~
The elements of of $\overrightarrow{\nabla Y^{(t)}}$ 
that are used in computing $\overrightarrow{\nabla X^{(t)}}[i,j]$ 
are identified and verified based on $Tree(\overrightarrow{\nabla Y})$.
According to Equation~(\ref{eq:conv-backward-1}), 
these elements include every $\overrightarrow{Y^{(t)}}[u,v]$ such that 
$u,v\in[\alpha_Y]$ and $i-u,j-v\in[n_F]\}$.
Also, these elements belong to every row $r$ of matrix $\overrightarrow{Y^{(t)}}$
such that $u\in[\alpha_Y]$ and $i-u\in[\alpha_F]$;
note that, the number of such rows is at most $\alpha_F$.
Thus, the TLM should retrieve all the elements in these rows. 
For each row $u$, it computes the hash value $h$ of all the elements in the row,
and checks if $h$ equals to the leaf node of $Tree(\overrightarrow{\nabla Y})$
with index $ind$ that corresponds to the row. 
If so, the co-path hash values of the leaf are retrieved and recorded as $e$, and
$Verify\_Commit(h,ind,comm(\overrightarrow{\nabla Y}),e)$ is called to 
verify the validity of the row.

{\noindent\em [Test~3]}:~
Lastly, $\overrightarrow{\nabla X^{(t)}}[i,j]$ is re-computed according to Equation~(\ref{eq:conv-backward-1})
and it is checked if the re-computed result equals to $\overrightarrow{\nabla X^{(t)}}[i,j]$
already verified in Test~1. \\


{\noindent\bf\underline{Selective Testing of $\overrightarrow{\nabla F}$}}:
The TLM randomly selects $p$ elements of $\overrightarrow{\nabla F}$ to test.
For each of the selected element,
denoted as $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$ for 
some $t\in[n_R]$ and $i,j,u\in[\alpha_F]$, 
the testing is as follows.

{\noindent\em [Test~1]}:~
The validity of $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$ is verified based on $Tree(\overrightarrow{\nabla F})$.
Specifically, 
the hash $h$ of all elements in vector $\overrightarrow{\nabla F^{(t)}_{i,j}}$ is computed;
the index $ind$ of the leaf node corresponding to $h$ in $Tree(\overrightarrow{\nabla F})$ is identified;
the co-path values for the leaf node are identified in $Tree(\overrightarrow{\nabla F})$ to form evidence $evid$;
$Verify\_Commit(h,ind,comm(\overrightarrow{\nabla F},evid)$ is called to 
verify the validity of the vector and thus its element $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$.

{\noindent\em [Test~2]}:~
The validity of $\overrightarrow{\nabla Y^{(t)}}[u]$, the row of matrix $\overrightarrow{\nabla Y^{(t)}}$ 
used in the computation of $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$ according to Equation~(\ref{eq:nabla_Ft_iju}),
is verified. Specifically,
the hash $h$ of all elements in $\overrightarrow{\nabla Y^{(t)}}[u]$ is computed;
the index $ind$ of the leaf node corresponding to $h$ in $Tree(\overrightarrow{\nabla Y})$ is identified;
the co-path values for the leaf node are identified in $Tree(\overrightarrow{\nabla Y})$ to form evidence $evid$;
$Verify\_Commit(h,ind,comm(\overrightarrow{\nabla F},evid)$ is called to 
verify the validity of $\overrightarrow{\nabla Y^{(t)}}[u]$.

{\noindent\em [Test~3]}:~
The validity of the group of $\vec{X}$, 
i.e., $\vec{X}_{i,j,u}=\{ \vec{X}[(u-1)\alpha_F+i,(v-1)\alpha_F+j] | v\in[n \}$,
is verified based on $Tree'(\vec{X})$. Specifically,
the hash $h$ of all elements in group $\vec{X}_{i,j,u}$ is computed;
the index $ind$ of the leaf node corresponding to $h$ in $Tree'(\vec{X})$ is identified;
the co-path values for the leaf node are identified in $Tree'(\vec{X})$ to form evidence $evid$;
$Verify\_Commit(h,ind,comm(\overrightarrow{\nabla F},evid)$ is called to 
verify the validity of group $\vec{X}_{i,j,u}$.

{\noindent\em [Test~4]}:~
Lastly, $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$ is re-computed according to Equation~(\ref{eq:nabla_Ft_iju})
and it is checked if the re-computed result equals to $\overrightarrow{\nabla F^{(t)}_{i,j}}[u]$
already verified in Test~1. \\

\comment{
Before the backward propagation starts, 
the UW should have already computed $\overrightarrow{\nabla Y^{(l)}}$
(i.e., the gradients for the inputs to layer $l$) and Merkle hash tree $MT(\overrightarrow{\nabla Y^{(l)}})$,
which includes the commitment $comm(\overrightarrow{\nabla Y^{(l)}})$ and the evidences
to verify each of the gradients. Also, 
the TLM should have received $comm(\overrightarrow{\nabla Y^{(l)}})$.


The backward propagation has two functions.
One is to compute the gradients for the outputs of layer $l-1$, i.e.,
$\overrightarrow{\nabla X^{(l-1)}}$, from $\overrightarrow{\nabla Y^{(l)}}$.
This is similar to the forward propagation 
elaborated in Section~\ref{sec:conv-forward-detail},
with only one slight difference that, 
the forward propagation is to compute $\overrightarrow{Y^{(l)}}$ from $\overrightarrow{ X^{(l-1)}}$
but the backward propagation is to compute 
$\overrightarrow{\nabla X^{(l-1)}}$ from $\overrightarrow{\nabla Y^{(l)}}$.
Hence, we will not step into the detail.

The other function is to compute the updates for the filters,
which is presented in the following. 

\subsubsection{Computation by the UW}

If being honest,
the UW should compute the updates for every element of the filters
following Equation~(\ref{eq:conv-update}) in Section~\ref{sec:conv-basic}.
Let $\overrightarrow{\nabla F} = (\overrightarrow{\nabla F_1}, \cdots, \overrightarrow{\nabla F_{n_F}})$.
Following the general model presented in Section~\ref{sec:select-test-general-model},
the UW calls $Construct\_Commit(\overrightarrow{\nabla F})$ 
to obtain $comm(\overrightarrow{\nabla F})$
and send it to the TLM.




However, if the selective testing is only based on 
the above commitment, the overhead could be very high due to the following reasons.
First, as shown in Equation~(\ref{eq:conv-update}),
to compute each $\overrightarrow{\nabla F_i}[j]$ 
(i.e., an element of $\overrightarrow{\nabla F}$),
$2q$ elements from 
$\overrightarrow{X^{(l-1)}}$ or $\overrightarrow{Y^{(l)}}$ need to be used.
Hence, when testing the computation of $\overrightarrow{\nabla F_i}[j]$,
the TLM would have to call the $Verify\_Element$ for $2q$ times. 
Note that $2q=\frac{2|\overrightarrow{Y^{(l)}}|}{n_F}$ 
could be a large number when $\overrightarrow{Y^{(l)}}$ is large;
for example, considering a convolutional layer that processes 
an image of $128\times 128$ pixels with 
a filter of $8\times 8$ elements and 
a stride of $2$,
the image would be transformed to around $4096$ data items; 
in this case, to verify the computation of one gradient of the filter, 
$8192$ calls of $Verify\_Element$ would be needed.

To address the problem,
we propose an enhancement in the following,
which can help to reduce the number of verification calls made by the TLM to ${\cal O}(p)$. 
Recall that $p$ is a small-value parameter specifying the number of computation instances that 
should be checked for each SIMD computation. 
Specifically, the UW should further do the following:

First, it divides $\overrightarrow{\nabla Y^{(l)}}$ into $n_F\cdot\sqrt{q}$ sub-vectors 
each of $\sqrt{q}$ elements; here we assume $\sqrt{q}$ to be integer to simplify presentation.
That is, 
\[
\overrightarrow{\nabla Y^{(l)}} = (\vec{Y}_1, \cdots, \vec{Y}_{n_F\cdot\sqrt{q}}),
\]
where for each $i\in [n_F\cdot\sqrt{q}]$,
\[
\vec{Y}_i = (
\overrightarrow{\nabla Y^{(l)}}[(i-1)\sqrt{q}+1], 
\cdots,
\overrightarrow{\nabla Y^{(l)}}[i\cdot\sqrt{q}]
).
\]
Then it calls $Construct\_Commit((\vec{Y}_1$, $\cdots$, $\vec{Y}_{n_F\cdot\sqrt{q}}))$
to build an additional Merkle hash tree for $\overrightarrow{\nabla Y^{(l)}}$,
denoted as $MT'(\overrightarrow{\nabla Y^{(l)}})$, 
where the hashes of every vectors $\vec{Y}_i$
instead of individual numbers are the leaf nodes. 
The root of the tree is denoted as $comm'(\overrightarrow{\nabla Y^{(l)}})$
to differentiate it from the commitment previously constructed with 
$Construct\_Commit(\overrightarrow{\nabla Y^{(l)}})$.

Second, the UW defines $\sqrt{q}$ sub-vectors of $\overrightarrow{X^{(l-1)}}$
denoted as $\vec{X}_1,\cdots,\vec{X}_{\sqrt{q}}$ such that
each $\vec{X}_i$ contains all the elements of $\overrightarrow{X^{(l-1)}}$
that are needed to compute 
$\overrightarrow{Y^{(l)}}[(i-1)\sqrt{q}+1]$,
$\cdots$, 
$\overrightarrow{Y^{(l)}}[i\cdot\sqrt{q}]$.
Formally, 
\[
\vec{X}_i = \bigcup_{j=(i-1)\sqrt{q}+1,\cdots,i\cdot\sqrt{q}}\phi_X(j).
\]
Hence, it holds that
\[
\overrightarrow{X^{(l-1)}} = \bigcup_{i\in[\sqrt{q}]}\vec{X}_i.
\]
Then, as in the above step,
it calls $Construct\_Commit(\vec{X}_1$, $\cdots$, $\vec{X}_{\sqrt{q}})$
to build an additional Merkle hash tree for $\overrightarrow{\nabla X^{(l-1)}}$,
denoted as $MT'(\overrightarrow{\nabla X^{(l-1)}})$, 
where the hashes of every vectors $\vec{X}_i$.
It denote the root of the tree as $comm'(\overrightarrow{\nabla X^{(l-1)}})$.

Third, the UW defines a vector $\overrightarrow{F'}_{i,j}$ for 
each element $\overrightarrow{F_i}[j]$ where $i\in [n_F]$ and $j\in [s_F]$.
$\overrightarrow{F'}_{i,j}$ has $\sqrt{q}$ elements and 
it has the following properties:
First, for each $k\in[\sqrt{q}]$,
$\overrightarrow{F'}_{i,j}[k]$ is computed from 
$\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$ and 
$\phi_X((k-1)\sqrt{q}+u)$ which is 
completely included in $\vec{X}_k$;
that is, computing or testing $\overrightarrow{F'}_{i,j}[k]$
only needs to access $\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$ and $\vec{X}_k$.
Second, the sum of all the $\sqrt{q}$ elements in $\overrightarrow{F'}_{i,j}$
is equal to $\overrightarrow{\nabla F_i}[j]$
as computed by Equation~(\ref{eq:conv-update}).
Formally, 
\[
\overrightarrow{F'}_{i,j}[k] = \sum_{u\in\sqrt{q}}\vec{Y}_{(i-1)\cdot\sqrt{q}+k}[u]\cdot\phi_X((k-1)\sqrt{q}+u)[j]. 
\]
Then, the UW calls $Construct\_Commit(\overrightarrow{F'}_{1,1}$, $\cdots$, $\overrightarrow{F'}_{n_F,s_F})$
to build an additional Merkle hash tree for $\overrightarrow{\nabla F}$,
denoted as $MT'(\overrightarrow{\nabla F})$,
where the hashes of every vectors $\overrightarrow{F'}_{i,j}$.
It denotes the root of the tree as $comm'(\overrightarrow{\nabla F})$.

At the end,
the UW sends the commitments 
$comm'(\overrightarrow{\nabla Y^{(l)}})$,
$comm'(\overrightarrow{\nabla X^{(l-1)}})$ and
$comm'(\overrightarrow{\nabla F})$ to the TLM. 
















\subsubsection{Selective Testing by the TLM}
After receiving the above commitments from the UW,
the TLM launches to test the computation of $p$ randomly selected elements of $\overrightarrow{\nabla F}$.
For each selected element denoted as $\overrightarrow{\nabla F_i}[j]$,
it first requests the UW for the following information:
(i) the value of $\overrightarrow{\nabla F_i}[j]$;
(ii) the evidence $evid_1$ for verifying the above value based on $comm(\overrightarrow{\nabla F}))$;  
(iii) vector $\overrightarrow{F'}_{i,j}$ which is leaf node on $MT'(\overrightarrow{\nabla F})$ 
that corresponds to $\overrightarrow{\nabla F_i}[j]$;
(ii) the evidences $evid_2$ for verifying $\overrightarrow{F'}_{i,j}$ based on $comm'(\overrightarrow{\nabla F})$.
Upon receiving the above, 
it conducts the following test:
\begin{itemize}
    \item 
    It tests if the sum of elements in $\overrightarrow{F'}_{i,j}$ equals to $\overrightarrow{\nabla F_i}[j]$.
    \item
    It calls $Verify\_Element(\overrightarrow{\nabla F_i}[j], i\cdot s_F+j, comm(\overrightarrow{\nabla F})), evid_1)$ 
    to verify if $\overrightarrow{\nabla F_i}[j]$ is a leaf node on $MT(\overrightarrow{\nabla F})$.
    \item 
    It calls $Verify\_Element(\overrightarrow{F'}_{i,j}, i\cdot s_F+j, comm'(\overrightarrow{\nabla F})), evid_2)$ 
    to verify if $\overrightarrow{F'}_{i,j}$ is a leaf node on $MT'(\overrightarrow{\nabla F})$.
\end{itemize}
If any of the tests fails, the UW is found dishonest;
otherwise, the testing continues as follows.

Second, the TLM randomly picks $p$ element in vector $\overrightarrow{F'}_{i,j}$ to test.
For each selected element denoted as $\overrightarrow{F'}_{i,j}[k]$,
it identifies that $\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$ and $\vec{X}_k$ are 
the sub-vectors of $\overrightarrow{\nabla Y^{(l)}}$ and $\overrightarrow{\nabla X^{(l-1)}}$
needed to compute $\overrightarrow{F'}_{i,j}[k]$.
Then, it requests the UW for:
(i) vector $\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$;
(ii) the evidence $evid_3$ for verifying the above value based on $comm'(\overrightarrow{\nabla Y^{(l)}})$;
(iii) vector $\vec{X}_k$;
(iv) the evidence $evid_4$ for verifying the above value based on $comm'(\overrightarrow{\nabla X^{(l-1)}})$;
(v) for an element $y$ randomly picked from $\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$, 
the evidence $evid_5$ for verifying $y$ to be a leaf node based on $comm(\overrightarrow{\nabla Y^{(l)}})$;
(vi) for an element $x$ randomly picked from $\vec{X}_k$, 
the evidence $evid_6$ for verifying $x$ to be a leaf node based on $comm(\overrightarrow{\nabla X^{(l-1)}})$.
Upon receiving the above,
the TLM tests the validity of the above
$\vec{Y}_{(i-1)\cdot\sqrt{q}+k}$, $y$ and $x$, respectively.
If any of the tests fails, the UW is found dishonest.

}



\subsection{Fully-connected Layer: Forward Propagation}

If the general model in Section~\ref{sec:select-test-general-model} is used,
when testing the computation of $\overrightarrow{Y}$ in the forward propagation through a fully-connected layer $l$, 
the TLM has to test the validity of the whole $\overrightarrow{X}$ and 
multiply it with $p$ randomly-selected columns of $\Theta$.
Similarly, when testing the computation of backward propagation through the layer,
the TLM has to test the validity of the whole $\overrightarrow{Y}$ and 
multiply it with $p$ randomly-selected rows of matrix $\Theta$. 
These could incur large overhead when $\overrightarrow{X}$ or $\overrightarrow{Y}$ has large size. 

For reduced cost,
we propose a hierarchical scheme,
in which the $l_X$-element vector $\vec{X}=(\vec{X}[1],\cdots,\vec{X}[l_X])$ 
is divided into $n_X$ sub-vectors each of $s_X$ elements. Here, 
$n_X\cdot s_X=l_X$, $n_X\approx\sqrt{l_X}$ and 
each sub-vector $\vec{X}_i=(\vec{X}[(i-1)\cdot s_X+1],\cdots,\vec{X}[i\cdot s_X])$ for each $i\in[n_X]$.  
Accordingly, the $l_Y$-element vector $\vec{Y}$ is expanded by $n_X$ times to 
obtain a $(l_Y,n_X)$ matrix $\overrightarrow{Y'}$,
such that $\vec{Y}[i]=\sum_{j\in [n_X]}\overrightarrow{Y'}[i,j]$.

\subsubsection{Computation by the UW}

For each $i\in[l_Y]$ and each $j\in[n_X]$,
the UW computes $\overrightarrow{Y'}[i,j]$ as follows:
\begin{equation}\label{eq:Y'_i_j}
    \overrightarrow{Y'}[i,j] = 
        \sum_{u\in[s_X]}\vec{X}[(j-1)s_X+u]\cdot \Theta[(j-1)s_X+u,i].
\end{equation}

For every $i\in[l_Y]$,
a hash of elements 
$\overrightarrow{Y'}[i,1],\cdots,\overrightarrow{Y'}[i.n_X]$
is computed.
Then, all of the afore-computed hash values are used as leaf nodes
to construct Merkel hash tree denoted as $Tree(\vec{Y})$.

For every sub-vector $\vec{X}_i$ of vector $\vec{X}$,
a hash of elements in the sub-vector is computed.
Then, all of the afore-computed hash values are used as leaf nodes
to construct Merkel hash tree denoted as $Tree(\vec{X})$.

$\Theta$, which is a $l_X\times l_Y$ matrix,
is divided into $n_X\times l_Y$ groups.
Every group $(i,j)$ contains elements
$\Theta[(i-1)s_X+1,\cdots,i\cdot s_X]$. 
Then, the hash for the elements of every group $(i,j)$ is computed,
and all of these hash values are used as leaf nodes
to construct a Merkel hash tree denoted as $Tree(\Theta)$.

Once $Tree(\vec{Y})$, $Tree(\vec{X})$ and $Tree(\Theta)$ have been constructed,
the roots of these trees, 
denoted as $comm(\vec{Y})$, $comm(\vec{X})$ and $comm(\Theta)$,
are sent to the TLM as commitments. 
Also, we assume that the UW also obtains a signature of $comm(\Theta)$ 
signed by the CS when it downloads the model from the CS;
the signature should be sent to the TLM as well. 

\subsubsection{Selective Testing by the TLM}

The UW provides the following information to the TLM:
(i) $\Theta$ and the signature of it signed by the CS; 
(ii) the pointers to the memory spaces where 
$\vec{X}$, $\overrightarrow{Y'}$, $\Theta$
$Tree(\vec{Y})$, $Tree(\vec{X})$ and $Tree(\Theta)$ are stored.
Upon receiving the above information,
the TLM randomly selects $p$ elements of matrix $\overrightarrow{Y'}$ to test. 
For each of the selected element, 
denoted as $\overrightarrow{Y'}[i,j]$,
the testing is conducted as follows.

{\noindent\em [Test~1]}:~
The validity of $\overrightarrow{Y'}[i,j]$ is tested based on 
$Tree(\vec{Y})$. 

{\noindent\em [Test~2]}:~
The validity of $\vec{X}_i$, 
which is used in computing $\overrightarrow{Y'}[i,j]$, 
is tested based on $Tree(\vec{X})$.

{\noindent\em [Test~3]}:~
The validity of group $(i,j)$ of $\Theta$, 
which is used in computing $\overrightarrow{Y'}[i,j]$,
is tested based on $Tree(\Theta)$. 

{\noindent\em [Test~4]}:~
$\overrightarrow{Y'}[i,j]$ is re-computed 
according to Equation~(\ref{eq:Y'_i_j}),
and then it is checked if the re-computed value equals to 
$\overrightarrow{Y'}[i,j]$ verified in Test~1.


\subsection{Fully-connected Layer: Backward Propagation}

The backward propagation procedure is similar to the forward propagation procedure.






\comment{


To support the design,
each TLM shares with the CS a pair of public/private key 
for certain partial homomorphic encryption (PHE) algorithm 
such as the Paillier Cryptosystem.

\subsubsection{Information Downloaded with Model}

At the beginning of each round, 
for each UW and its co-located TLM who requests to download the current model of neural network,
the CS should prepare and provide some material in addition to the model. 
Specifically, 
for each fully-connected layer $l$, 
the CS prepares the material as follows.

First, it randomly generates two secret vectors: 
$\vec{f}_l$ of $n_l$ elements used for testing forward propagation and
$\vec{b}_l$ of $n_{l-1}$ elements used for testing backward propagation. 
Then, it derives two more secret vectors $\vec{f'}_l$ and $\vec{b'}_l$ as follows:
\begin{equation}
\vec{f'}_l\leftarrow \vec{f}_l\times  ({\Theta}^{(l)})^\intercal,~~
\vec{b'}_l\leftarrow \vec{b}_l\times  {\Theta}^{(l)}.
\end{equation}
Note that, $\vec{f}_l$, $\vec{b}_l$, $\vec{f'}_l$ and $\vec{b'}_l$ are all row vectors;
$\vec{f}_l$ and $\vec{b'}_l$ each has $n_l$ elements
while $\vec{b}_l$ and $\vec{f'}_l$ each has $n_{l-1}$ elements.

Second, from each of these vectors, the CS further derives 
a secret set of pairs and an PHE-encrypted vector. 
Taking $\vec{f}_l$ as example, we explain the derivation in the following. 
\begin{itemize}

\item 
The CS randomly selects $p$ elements from $\vec{f}_l$ to form 
a secret set of pairs, denoted as 
\[
SF_l=\{(i_1,\vec{f}_l[i_1]), \cdots, (i_p,\vec{f}_l[i_p])\}
\]
where each pair $(i_j,\vec{f}_l[i_j])$ records 
a randomly selected element in $\vec{f}_l$ and 
its index in the vector. 

\item 
The CS constructs an PHE-encrypted vector, 
denoted as $\overrightarrow{phe(f)}_l$ 
according to the rule as follows:
for each $j\in [n_l]$,
    \begin{equation}
        \overrightarrow{phe(f)}_l[j] = 
            \begin{cases}
                phe(0) & (j,\vec{f}_j)\in SF_l\\
                phe(\vec{f}_l[j]) & \textit{otherwise}.
            \end{cases}
    \end{equation}
\end{itemize}
In the similar manner,
$SF'_l$ and $\overrightarrow{phe(f')}_l$ can be constructed from $\vec{f'}_l$;
$SB_l$ and $\overrightarrow{phe(b)}_l$ can be constructed from $\vec{b}_l$; and
$SB'_l$ and $\overrightarrow{phe(b')}_l$ can be constructed from $\vec{b'}_l$.

After the above have been constructed,
the CS provides to each UW the following information along with the current model of the neural network:
\begin{equation}
\overrightarrow{phe(f)}_l,~
\overrightarrow{phe(f')}_l,~
\overrightarrow{phe(b)}_l,~\text{and}~
\overrightarrow{phe(b')}_l
\end{equation}
for each layer $l$. 
It provides to each TLM the following information
\begin{equation}
SF_l,~SF'_l,~SB_l,~\text{and}~SB'_l
\end{equation}
encrypted with the pairwise key shared with the TLM, 
for each layer $l$.


\subsubsection{Forward Propagation}

For fully-connected layer $l$,
the TLM interacts with the UW as follows 
to test the forward propagation from $\overrightarrow{X^{(l-1)}}$ to $\overrightarrow{Y^{(l)}}$.

    
    Following the general model in Section~\ref{sec:select-test-general-model}, 
    the UW first computes $\overrightarrow{Y^{(l)}}$,
    calls $Construct\_Commit(\overrightarrow{Y^{(l)}})$ to built a Merkle hash tree and obtain $comm(\overrightarrow{Y^{(l)}})$, 
    and sends $comm(\overrightarrow{Y^{(l)}})$ to the TLM.
    In addition, the UW computes:
    \begin{equation}
        phe(\beta_l) = \overrightarrow{X^{(l-1)}}\cdot \overrightarrow{phe(f')}_l
    \end{equation}
    and
    \begin{equation}
        phe(\gamma_l) = \overrightarrow{Y^{(l)}}\cdot \overrightarrow{phe(f)}_l.
    \end{equation}
    Note that, $phe(\beta_l)$ and $phe(\gamma_l)$ are notations we introduce here to 
    indicate that they are PHE ciphertexts.
    These results are also submitted to the TLM.
    

    Upon receiving the above, 
    the TLM retrieves and verifies the validity of 
    the elements of $\overrightarrow{X^{(l-1)}}$
    whose indices are in $SF'_l$
    and the elements of $\overrightarrow{Y^{(l)}}$
    whose indices are in $SF_l$.
    Specifically, for each $(j,f'_l[j])\in SF'_l$,
    the TLM requests the UW for $\overrightarrow{X^{(l-1)}}[j]$ and its associated evidence $evid$,
    and then calls $Verify\_Element(\overrightarrow{X^{(l-1)}}[j], j, commit(\overrightarrow{X^{(l-1)}}), evid)$
    to verify the validity of the element. 
    The retrieval and verification of the elements in $\overrightarrow{Y^{(l)}}$ is similar.
    
    

    Finally, the TLM decrypts $phe(\beta_l)$ and $phe(\gamma_l)$ to $\beta_l$ and $\gamma_l$ and 
    checks if the following equality holds:
    \begin{eqnarray}
        &&  \beta_l + \sum_{\forall (j,f'_l[j])\in SF'_l} \overrightarrow{X^{(l-1)}}[j]\cdot f'_l[j]\nonumber\\
        &=& \gamma_l + \sum_{\forall (j,f_l[j])\in SF_l} \overrightarrow{Y^{(l)}}[j]\cdot f_l[j].
    \end{eqnarray}
    If the equality holds, the testing succeeds;
    otherwise, the UW is found dishonest. 



\subsubsection{Backward Propagation}

To test the computation of $\overrightarrow{\nabla X^{(l-1)}}$ from $\overrightarrow{\nabla Y^{(l)}}$
is similar to the testing of forward propagation,
and so we skip it due to the limit in space. 

To test the computation of updates to $\Theta^{(l)}$,
the general model in Section~\ref{sec:select-test-general-model} can be applied directly.

}

    
    
    
    







==> enhanced_design.tex <==

\section{Enhancements for Higher Efficiency}

In this section,
we presents two enhancements to improve the efficiency
in testing the forward/backward propagation through a fully-connected layer
and the backward propagation through a convolutional layer. 


\subsection{Enhancements for Fully-connected Layer}

With the scheme proposed in the previous section, 
when testing the validity of input in a fully-connected layer $l$, 
the TLM has to multiply the whole output vector of layer $l-1$ 
with $\alpha$ selected rows of the transpose of matrix $\Theta^{(l)}$,
involving $O(n^2)$ number of multiplications. 
Similarly, when testing the validity of backward propagation through layer $l$,
the TLM has to multiply the whole input vector of the layer with $\alpha$ selected rows of matrix $\Theta^{(l)}$. 
To reduce the cost,
we propose the following enhancements.

For the simplicity of presentation, 
we first assume that only one piece of training data is used at each local worker for each round;
later we discuss how this can be extended to the case that multiple pieces of training data are used. 


To support these enhancements,
each TLM should share with the TA a pair of public/private key 
for partial homomorphic encryption (PHE) 
such as the Paillier cryptosystem.

\subsubsection{Information Downloaded with Model}

At the beginning of each round, 
for each UW and its co-located TLM who requests to download the current model of neural network,
the TA should prepare and provide some material in addition to the model. 
Specifically, 
for each fully-connected layer $l$, 
the TA prepares the material as follows.

First, it randomly generates two secret vectors: 
$\vec{f}_l$ of $n_l$ elements used for testing forward propagation and
$\vec{b}_l$ of $n_{l-1}$ elements used for testing backward propagation. 
Then, it derives two more secret vectors $\vec{f'}_l$ and $\vec{b'}_l$ as follows:
\begin{equation}
\vec{f'}_l\leftarrow \vec{f}_l\times  ({\Theta}^{(l)})^\intercal,~~
\vec{b'}_l\leftarrow \vec{b}_l\times  {\Theta}^{(l)}.
\end{equation}
Note that, $\vec{f}_l$, $\vec{b}_l$, $\vec{f'}_l$ and $\vec{b'}_l$ are all row vectors;
$\vec{f}_l$ and $\vec{b'}_l$ each has $n_l$ elements
while $\vec{b}_l$ and $\vec{f'}_l$ each has $n_{l-1}$ elements.

Second, from each of these vectors, the TA further derives 
a secret set of pairs and an PHE-encrypted vector. 
Taking $\vec{f}_l$ as example, we explain the derivation in the following. 
\begin{itemize}

\item 
The TA randomly selects $\alpha$ elements from $\vec{f}_l$ to form 
a secret set of pairs, denoted as 
\[
SF_l=\{(i_1,\vec{f}_l[i_1]), \cdots, (i_\alpha,\vec{f}_l[i_\alpha])\}
\]
where each pair $(i_1,\vec{s}_l[i_1])$ records 
a randomly selected element in $\vec{s}_l$ and its corresponding index in the vector. 

\item 
The TA constructs an PHE-encrypted vector, 
denoted as $\overrightarrow{phe(f)}_l$ 
according to the rule as follows:
for each $j\in [n_l]$,
    \begin{equation}
        \overrightarrow{phe(f)}_l[j] = 
            \begin{cases}
                phe(0) & (j,\vec{f}_j)\in SF_l\\
                phe(\vec{f}_l[j]) & \textit{otherwise}.
            \end{cases}
    \end{equation}
\end{itemize}
In the similar manner,
$SF'_l$ and $\overrightarrow{phe(f')}_l$ can be constructed from $\vec{f'}_l$;
$SB_l$ and $\overrightarrow{phe(b)}_l$ can be constructed from $\vec{b}_l$; and
$SB'_l$ and $\overrightarrow{phe(b')}_l$ can be constructed from $\vec{b'}_l$.

After the above have been constructed,
the TA provides to each UW the following information along with the current model of the neural network:
\begin{equation}
\overrightarrow{phe(f)}_l,~
\overrightarrow{phe(f')}_l,~
\overrightarrow{phe(b)}_l,~\text{and}~
\overrightarrow{phe(b')}_l
\end{equation}
for each layer $l$. 
It provides to each TLM the following information
\begin{equation}
SF_l,~SF'_l,~SB_l,~\text{and}~SB'_l
\end{equation}
encrypted with the pairwise key shared with the TLM, 
for each layer $l$.


\subsubsection{Forward Propagation}

For fully-connected layer $l$,
the TLM interacts with the UW as follows 
to test the forward propagation from the output of layer $l-1$ to the input of layer $l$.
\begin{itemize}
    \item 
    At this point, the UW should have already committed the output of layer $l-1$.
    As in the basic scheme, 
    we denote the output of layer $l-1$ as $\vec{o}_{l-1}$ and
    the commitment 
    (i.e., the root of Merkle tree with the hashes of elements of $\vec{o}_{l-1}$ as leaf nodes) 
    as $com(\vec{o}_{l-1})$. 
    
    \item 
    The UW computes the input to layer $l$,
    denoted as 
    $\vec{i}_l\leftarrow (\Theta^{(l)})^\intercal \times \vec{o}_{l-1}$,
    and commits the computation by constructing a Merkle tree with the hashes of the elements of $\vec{i}_l$ as leaf node
    and submits to the TLM the root of the tree,
    denoted as $com(\vec{i}_l)$.
    
    \item 
    The UW also computes:
    \begin{equation}
        phe(\beta_l) = \vec{o}_{l-1}\cdot \overrightarrow{phe(f')}_l
    \end{equation}
    and
    \begin{equation}
        phe(\gamma_l) = \vec{i}_{l}\cdot \overrightarrow{phe(f)}_l.
    \end{equation}
    These results are also submitted to the TLM.
    
    \item 
    Upon receiving $com(\vec{i}_l)$, $phe(\beta_l)$ and $phe(\gamma_l)$,
    the TLM retrieves the committed elements in $\vec{o}_{l-1}$ whose indices are in $SF'_l$
    and the committed elements in $\vec{i}_{l}$ whose indices are in $SF_l$.
    
    \item 
    The TLM decrypts $phe(\beta_l)$ and $phe(\gamma_l)$ to $\beta_l$ and $\gamma_l$ respectively.
    Then, it checks if the following equality holds:
    \begin{eqnarray}
        &&  \beta_l + \sum_{\forall (j,f'_l[j])\in SF'_l} \vec{o}_{l-1}[j]\cdot f'_l[j]\nonumber\\
        &=& \gamma_l + \sum_{\forall (j,f_l[j])\in SF_l} \vec{i}_{l}[j]\cdot f_l[j].
    \end{eqnarray}
    If the equality holds, the checking succeeds;
    otherwise, the UW is found misbehaving. 
\end{itemize}


\subsubsection{Backward Propagation}

The testing of the backward-propagating 
the input gradients of fully-connected layer $l$ to 
the output gradients of layer $l-1$ is similar to 
the afore-discussed forward propagation. 
The detail is as follows. 
\begin{itemize}
    \item 
    At this point, the UW should have already committed the input gradients of layer $l$.
    As in the basic scheme, 
    we denote the input gradients of layer $l$ as $\overrightarrow{\nabla i}_{l}$ and
    the commitment as $com(\overrightarrow{\nabla i}_{l})$. 
    
    \item 
    The UW computes the gradients of output of layer $l-1$,
    denoted as
    $\overrightarrow{\nabla o}_{l-1} \leftarrow \Theta^{(l)} \times \overrightarrow{\nabla i}_{l}$, 
    and commits the computation by constructing a Merkle tree with the hashes of the elements of 
    $\overrightarrow{\nabla o}_{l-1}$ as leaf node
    and submits to the TLM the root of the tree,
    denoted as $com(\overrightarrow{\nabla o}_{l-1})$.
    
    \item 
    The UW also computes:
    \begin{equation}
        phe(\beta'_l) = \overrightarrow{\nabla i}_{l}\cdot \overrightarrow{phe(f')}_l
    \end{equation}
    and
    \begin{equation}
        phe(\gamma'_l) = \overrightarrow{\nabla i}_{l}\cdot \overrightarrow{phe(f)}_l.
    \end{equation}
    Here, symbol $\cdot$ denotes the operation of inner product. 
    These results are also submitted to the TLM.
    
    \item 
    Upon receiving $com(\overrightarrow{\nabla o}_{l-1})$, $phe(\beta'_l)$ and $phe(\gamma'_l)$,
    the TLM retrieves the committed elements in $\vec{o}_{l-1}$ whose indices are in $SF'_l$
    and the committed elements in $\vec{i}_{l}$ whose indices are in $SF_l$.
    
    \item 
    The TLM decrypts $phe(\beta'_l)$ and $phe(\gamma'_l)$ to $\beta'_l$ and $\gamma'_l$ respectively.
    Then, it checks if the following equality holds:
    \begin{eqnarray}
        &&  \beta'_l + \sum_{\forall (j,b'_l[j])\in SB'_l} \vec{o}_{l-1}[j]\cdot b'_l[j]\nonumber\\
        &=& \gamma'_l + \sum_{\forall (j,b_l[j])\in SB_l} \vec{i}_{l}[j]\cdot b_l[j].
    \end{eqnarray}
    If the equality holds, the checking succeeds;
    otherwise, the UW is found misbehaving. 
\end{itemize}



\subsection{Enhancement for Convolutional Layer}

The backward propagation through a convolutional layer $l$ can be costly 
when the size of output from layer $l-1$ is very large. 

For example, ... 

The idea of our proposed enhancement is to organize the computation into a tree (hierarchy) and 
then only need to check the computation along a path ... 




